Data-Dependent Differentially Private Parameter Learning for Directed Graphical Models

Directed graphical models (DGMs) are a class of probabilistic models that are widely used for predictive analysis in sensitive domains, such as medical diagnostics. In this paper we present an algorithm for differentially private learning of the parameters of a DGM with a publicly known graph structure over fully observed data. Our solution optimizes for the utility of inference queries over the DGM and \textit{adds noise that is customized to the properties of the private input dataset and the graph structure of the DGM}. To the best of our knowledge, this is the first explicit data-dependent privacy budget allocation algorithm for DGMs. We compare our algorithm with a standard data-independent approach over a diverse suite of DGM benchmarks and demonstrate that our solution requires a privacy budget that is $3\times$ smaller to obtain the same or higher utility.

==> proof.tex <==
\begin{comment}




Additionally, we prove two lemmas here which will be used in proving the bounds in the following section.
\begin{lem} If the error for a sum-product term of the form, $\phi_A=\sum_{x}\prod_{i=1}^t\phi_i, t \in \{2,\cdots,n\}$ in the variable elimination algorithm where $X$ is the attribute being eliminated, is given by \begin{gather}\delta_{\phi_{\mathpzc{A}}} \geq\delta^{min}_{\phi_i[a,x]}\cdot\mathcal{C}\label{eq:refer1} \end{gather} where $\mathpzc{A}=\bigcup_{\phi_i}Attr(\phi_i)/X, x \in dom(X)$, $\delta^{min}_{\phi_i[a,x]}=min_{i,a,x}\{\delta_{\phi_i[a,x]}\}$ and some constant $\mathcal{C}<1$ then for the error of any marginal inference query, $\mathcal{Q}$ we have \begin{gather*}\delta_{\mathcal{Q}}\geq \delta \mathcal{C}^{n-1}\\ \delta=\min_{X_i}\{\min_{x_i,x_{pa_i}}\{\delta_{\Theta[x_i|x_{pa_i}]}\}\}\end{gather*}\label{lem:help1}\end{lem}
\begin{proof}We will prove the result via induction. \\  \textbf{Base Case:}\\ Let $\prec=\{X_1,X_2,\cdots,X_n\}$ be the order of elimination for the variable elimination algorithm. Clearly for the first sum-product term, $\phi_{\mathpzc{A}_1}=\sum_{x_1}\prod_{i=1}^t\phi^{X_1}_i, t \in \{2,\cdots,n\}, x_1 \in dom(X_1),\mathpzc{A}_1= \bigcup_{\phi_i}Attr(\phi^{X_1}_i)/X_1$ since all the factors $\phi_i, i \in [t]$ are actually true parameters of the DGM, $\Theta$, we have \begin{gather*}\delta^{min}_{\phi^{X_1}_i[a,x]}=\min_{X_i}\{\min_{x_i,x_{pa_i}}\{\delta_{\Theta[x_i|x_{pa_i}]}\}\}\end{gather*}
Now let us consider the computation of the second sum-product term,\begin{gather*}\phi_{\mathpzc{A}_2}=\sum_{x_2}\prod_{i=1}^t\phi^{X_2}_i,\mathpzc{A}_2= \bigcup_{\phi_i}Attr(\phi^{X_2}_i)/X_2 \end{gather*} Here all the factors $\phi^{X_2}_i \in \{\Theta \cup \phi_{\mathpzc{A}_2}\}$  and since $\mathcal{C} < 1$, clearly by eq \eqref{eq:refer1} we have\begin{gather*}\delta^{min}_{\phi^{X_2}_i[a,x]} \geq\delta_{\phi_{\mathpzc{A}_2}}\mathcal{C}\geq \delta\mathcal{C}^2 \end{gather*}
\\Since the answer of the marginal inference query $Q$ is the last sum-product term and there can be at most $n-1$ such terms,  by induction, it is evident that \begin{gather*}\delta_{\mathcal{Q}}\geq \delta\mathcal{C}^{n-1}\end{gather*}\end{proof}
\begin{lem}If the error for a sum-product term of the form, $\phi_A=\sum_{x}\prod_{i=1}^t\phi_i, t \in \{2,\cdots,n\}$ in the variable elimination algorithm where $X$ is the attribute being eliminated, is given by \begin{gather}\delta_{\phi_{\mathpzc{A}}} \leq\delta^{max}_{\phi_i[a,x]}\cdot\mathcal{C}\label{eq:refer2} \end{gather} where $\mathpzc{A}=\bigcup_{\phi_i}Attr(\phi_i)/X, x \in dom(X)$, $\delta^{max}_{\phi_i[a,x]}=max_{i,a,x}\{\delta_{\phi_i[a,x]}\}$ and some constant $\mathcal{C}>1$ then for the error of any marginal inference query, $\mathcal{Q}$ we have \begin{gather*}\delta_{\mathcal{Q}}\leq \delta \mathcal{C}^{n-1}\\ \delta=\max_{X_i}\{\max_{x_i,x_{pa_i}}\{\delta_{\Theta[x_i|x_{pa_i}]}\}\}\end{gather*}\label{lem:help2}\end{lem}
\begin{proof} The proof is very similar to that of Lemma \ref{lem:help1}. \textbf{Base Case:}\\ Let $\prec=\{X_1,X_2,\cdots,X_n\}$ be the order of elimination for the variable elimination algorithm. Clearly for the first sum-product term, $\phi_{\mathpzc{A}_1}=\sum_{x_1}\prod_{i=1}^t\phi^{X_1}_i, t \in \{2,\cdots,n\}, x_1 \in dom(X_1),\mathpzc{A}_1= \bigcup_{\phi_i}Attr(\phi^{X_1}_i)/X_1$ since all the factors $\phi_i, i \in [t]$ are actually true parameters of the DGM, $\Theta$, we have \begin{gather*}\delta^{max}_{\phi^{X_1}_i[a,x]}=\max_{X_i}\{\max_{x_i,x_{pa_i}}\{\delta_{\Theta[x_i|x_{pa_i}]}\}\}\end{gather*}
Now let us consider the computation of the second sum-product term,\begin{gather*}\phi_{\mathpzc{A}_2}=\sum_{x_2}\prod_{i=1}^t\phi^{X_2}_i,\mathpzc{A}_2= \bigcup_{\phi_i}Attr(\phi^{X_2}_i)/X_2 \end{gather*} Here all the factors $\phi^{X_2}_i \in \{\Theta \cup \phi_{\mathpzc{A}_2}\}$  and since $\mathcal{C} > 1$, clearly by eq \eqref{eq:refer2} we have\begin{gather*}\delta^{max}_{\phi^{X_2}_i[a,x]} \leq\delta_{\phi_{\mathpzc{A}_2}}\mathcal{C}\leq \delta\mathcal{C}^2 \end{gather*}
\\Since the answer of the marginal inference query $Q$ is the last sum-product term and there can be at most $n-1$ such terms,  by induction, it is evident that \begin{gather*}\delta_{\mathcal{Q}}\geq \delta\mathcal{C}^{n-1}\end{gather*} \end{proof}




\end{comment}
